Parallel and External-Memory Construction of Minimal Perfect Hash Functions with PTHash

A function $f : U \to \{0,\ldots,n-1\}$ is a minimal perfect hash function for a set $S \subseteq U$ of size $n$, if $f$ bijectively maps $S$ into the first $n$ natural numbers. These functions are important for many practical applications in computing, such as search engines, computer networks, and databases. Several algorithms have been proposed to build minimal perfect hash functions that: scale well to large sets, retain fast evaluation time, and take very little space, e.g., 2 - 3 bits/key. PTHash is one such algorithm, achieving very fast evaluation in compressed space, typically several times faster than other techniques. In this work, we propose a new construction algorithm for PTHash enabling: (1) multi-threading, to either build functions more quickly or more space-efficiently, and (2) external-memory processing to scale to inputs much larger than the available internal memory. Only few other algorithms in the literature share these features, despite of their big practical impact. We conduct an extensive experimental assessment on large real-world string collections and show that, with respect to other techniques, PTHash is competitive in construction time and space consumption, but retains 2 - 6$\times$ better lookup time.

==> tables/compression.10e9.a099.mphf_xor.tex <==

\begin{tabular}{c c ccccccc}
\toprule

  \multirow{2}{*}{$c$}
& \multirow{2}{*}{constr. (secs)}
& \multicolumn{7}{c}{{space (\bpk)}} \\


\cmidrule(lr){3-9}

&
& C
& C-C
& D
& D-D
& D-EF
& EF
& SDC
\\

\cmidrule(lr){1-9}

6 & 1799 & \cellcolor{white}{3.10} & \cellcolor{white}{2.96} & \cellcolor{white}{2.90} & \cellcolor{white}{2.84} & \cellcolor{white}{2.36} & \cellcolor{white}{2.17} & \cellcolor{white}{2.23} \\

7 & 1042 & \cellcolor{white}{3.14} & \cellcolor{white}{3.14} & \cellcolor{white}{3.14} & \cellcolor{white}{3.07} & \cellcolor{white}{2.50} & \cellcolor{white}{2.27} & \cellcolor{white}{2.31} \\

8 & 745 & \cellcolor{white}{3.57} & \cellcolor{white}{3.49} & \cellcolor{white}{3.30} & \cellcolor{white}{3.30} & \cellcolor{white}{2.68} & \cellcolor{white}{2.39} & \cellcolor{white}{2.41} \\

9 & 589 & \cellcolor{white}{3.70} & \cellcolor{white}{3.70} & \cellcolor{white}{3.40} & \cellcolor{white}{3.40} & \cellcolor{white}{2.78} & \cellcolor{white}{2.47} & \cellcolor{white}{2.47} \\

10 & 512 & \cellcolor{white}{4.11} & \cellcolor{white}{4.01} & \cellcolor{white}{3.77} & \cellcolor{white}{3.67} & \cellcolor{white}{2.87} & \cellcolor{white}{2.59} & \cellcolor{white}{2.53} \\

11 & 449 & \cellcolor{white}{4.14} & \cellcolor{white}{4.14} & \cellcolor{white}{4.14} & \cellcolor{white}{4.03} & \cellcolor{white}{3.01} & \cellcolor{white}{2.67} & \cellcolor{white}{2.59} \\


\cmidrule(lr){1-9}

\multicolumn{2}{c}{lookup ({\nspk})}
 & 37 & 37 & 49 & 49 & 75 & 101 & 170 \\

\bottomrule
\end{tabular}



==> tables/compression.10e9.mphf_xor.tex <==

\begin{tabular}{c c ccccccc}
\toprule

  \multirow{2}{*}{$c$}
& \multirow{2}{*}{constr. (secs)}
& \multicolumn{7}{c}{{space (\bpk)}} \\


\cmidrule(lr){3-9}

&
& C
& C-C
& D
& D-D
& D-EF
& EF
& SDC
\\

\cmidrule(lr){1-9}

6 & 2415 & \cellcolor{white}{6.02} & \cellcolor{white}{5.60} & \cellcolor{white}{3.21} & \cellcolor{white}{3.03} & \cellcolor{white}{2.39} & \cellcolor{white}{2.22} & \cellcolor{white}{2.22} \\

7 & 1578 & \cellcolor{white}{7.49} & \cellcolor{white}{6.23} & \cellcolor{white}{3.75} & \cellcolor{white}{3.54} & \cellcolor{white}{2.66} & \cellcolor{white}{2.41} & \cellcolor{white}{2.31} \\

8 & 1150 & \cellcolor{white}{8.03} & \cellcolor{white}{6.66} & \cellcolor{white}{4.28} & \cellcolor{white}{3.96} & \cellcolor{white}{2.82} & \cellcolor{white}{2.58} & \cellcolor{white}{2.39} \\

9 & 993 & \cellcolor{white}{9.33} & \cellcolor{white}{7.62} & \cellcolor{white}{4.82} & \cellcolor{white}{4.37} & \cellcolor{white}{3.02} & \cellcolor{white}{2.78} & \cellcolor{white}{2.47} \\

10 & 913 & \cellcolor{white}{10.37} & \cellcolor{white}{9.97} & \cellcolor{white}{5.35} & \cellcolor{white}{5.05} & \cellcolor{white}{3.48} & \cellcolor{white}{2.99} & \cellcolor{white}{2.53} \\

11 & 813 & \cellcolor{white}{10.67} & \cellcolor{white}{10.12} & \cellcolor{white}{5.89} & \cellcolor{white}{5.56} & \cellcolor{white}{3.75} & \cellcolor{white}{3.19} & \cellcolor{white}{2.60} \\


\cmidrule(lr){1-9}

\multicolumn{2}{c}{lookup ({\nspk})}
 & 36 & 36 & 49 & 48 & 73 & 96 & 165 \\

\bottomrule
\end{tabular}



==> tables/ext_mem/EMPHF_partitioned.tex <==
% !TEX root = ../../paper.tex
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

TweetsKB IDs
& 909 & 3.03 & 279 \\
%before: & 1204 & 3.03 & 279 \\

ClueWeb09-Full URLs
& 3980 & 3.31 & 304 \\
%before: & 6853 & 3.31 & 304 \\

GoogleBooks 3-gr
& 5606 & 3.06 & 304 \\
%before: & 6971 & 3.06 & 311 \\

\bottomrule
\end{tabular}


==> tables/ext_mem/EMPHF_single.tex <==
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

TweetsKB IDs
& 3200 & 2.61 & 207 \\
% query time is measured by executing 100M queries
% using the program ./test_mphf

GoogleBooks 3-gr
& 37255 & 2.61 & 225 \\
% query time is measured by executing 200M queries
% using the program ./test_mphf

\bottomrule
\end{tabular}


==> tables/ext_mem/GOV_single.tex <==
% !TEX root = ../../paper.tex
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

TweetsKB IDs
& {1796} & {2.23} & {\e} \\
GoogleBooks 3-gr
& {\e} & {\e} & {\e} \\

\bottomrule
\end{tabular}


==> tables/ext_mem/PTHash_partitioned.tex <==
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

TweetsKB IDs
& {\e} & {\e} & {\e} \\

ClueWeb09-Full URLs
& {\e} & {\e} & {\e} \\

GoogleBooks 3-gr
& {\e} & {\e} & {\e} \\

\bottomrule
\end{tabular}


==> tables/ext_mem/PTHash_single.tex <==
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

% {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "557.798000", "searching_seconds": "1498.549000", "encoding_seconds": "11.023000", "total_seconds": "2067.370000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "85.628975"}
TweetsKB IDs
& 2068 & 3.07 & 86 \\

% {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "2100.912000", "searching_seconds": "6986.289000", "encoding_seconds": "35.983000", "total_seconds": "9123.184000", "pt_bits_per_key": "2.498342", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "110.384842"}
GoogleBooks 3-gr
& 9123 & 2.91 & 110 \\

\bottomrule
\end{tabular}


==> tables/ext_mem/parallel.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c ccc c ccc c ccc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{3}{c}{TweetsKB IDs}
&& \multicolumn{3}{c}{ClueWeb09-Full URLs}
&& \multicolumn{3}{c}{GoogleBooks 3-gr} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

{\pth} (D-D, $\alpha=0.94$, $c=7.0$)
&& 555 & 2.85 & 118
&& 2789 & 2.75 & 156
&& 2407 & 2.71 & 138 \\


{\pth} (PC, $\alpha=0.94$, $c=7.0$)
&& 555 & 2.61 & 132
&& 2787 & 2.58 & 193
&& 2403 & 2.57 & 189 \\

\midrule

GOV
&& 1463 & 2.23 & 192
&& 5400 & 2.23 & 232
&& 6461 & 2.23 & 242 \\

\midrule

BBHash ($\gamma=1.0$)
&& 931 & 3.07 & 294
&& 18391 & 3.07 & 320
&& 9554 & 3.07 & 305 \\

BBHash ($\gamma=2.0$)
&& 590 & 3.71 & 217
&& 10348 & 3.71 & 236
&& 5404 & 3.71 & 235 \\


\bottomrule
\end{tabular}

==> tables/ext_mem/partitioned.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c ccc c ccc c ccc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{3}{c}{TweetsKB IDs}
&& \multicolumn{3}{c}{ClueWeb09-Full URLs}
&& \multicolumn{3}{c}{GoogleBooks 3-gr} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

{\pth} (D-D, $\alpha=0.94$, $c=7.0$)
&& 999 & 2.85 & 117
&& 4384 & 2.75 & 152
&& 5055 & 2.71 & 135 \\

{\pth} (PC, $\alpha=0.94$, $c=7.0$)
&& 993 & 2.61 & 131
&& 4369 & 2.58 & 191
&& 5030 & 2.57 & 187 \\

{\pth} (EF, $\alpha=0.94$, $c=7.0$)
&& 994 & 2.36 & 204
&& 4371 & 2.32 & 236
&& 5034 & 2.31 & 228 \\

\midrule


EMPHF-HEM
&& 909 & 3.03 & 279
%before: & 1204 & 3.03 & 279 \\

&& 3980 & 3.31 & 304
%before: & 6853 & 3.31 & 304 \\

&& 5606 & 3.06 & 304 \\
%before: & 6971 & 3.06 & 311 \\

\bottomrule
\end{tabular}

==> tables/ext_mem/single.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c ccc c ccc c ccc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{3}{c}{TweetsKB IDs}
&& \multicolumn{3}{c}{ClueWeb09-Full URLs}
&& \multicolumn{3}{c}{GoogleBooks 3-gr} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

{\pth} (D-D, $\alpha=0.94$, $c=7.0$)


% the following results are taken without multi-threading nor async threads
% {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partit
% ioning_seconds": "0.000000", "mapping_ordering_seconds": "754.962000", "searching_seconds": "1622.231000", "encoding_seconds": "11.476000", "total_seconds": "2388.669000", "pt_bits_per_key": "2.6517
% 74", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "0.000000"}
% {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "5029.884000", "searching_seconds": "4700.373000", "encoding_seconds": "23.693000", "total_seconds": "9753.950000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "0.000000"}
% {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3644.393000", "searching_seconds": "7616.943000", "encoding_seconds": "36.220000", "total_seconds": "11297.556000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "0.000000"}

% below is new version with 1 pass over the input
% {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "716.701000", "searching_seconds": "1496.442000", "encoding_seconds": "11.241000", "total_seconds": "2224.384000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "0.000000"}
% {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3587.340000", "searching_seconds": "4380.904000", "encoding_seconds": "23.547000", "total_seconds": "7991.791000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "0.000000"}
% {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3520.978000", "searching_seconds": "7529.102000", "encoding_seconds": "35.901000", "total_seconds": "11085.981000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "0.000000"}

% below is new version with 1 pass over the input [Rob]
%{"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "718.687000", "searching_seconds": "1314.088000", "encoding_seconds": "11.592000", "total_seconds": "2044.367000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "0.000000"}
%{"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3686.328000", "searching_seconds": "3690.745000", "encoding_seconds": "24.398000", "total_seconds": "7401.471000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "0.000000"}
%{"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3876.872000", "searching_seconds": "6133.358000", "encoding_seconds": "37.308000", "total_seconds": "10047.538000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "0.000000"}


% latest results [revised Rob version]
% {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "673.557000", "searching_seconds": "1350.255000", "encoding_seconds": "11.613000", "total_seconds": "2035.425000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "0.000000"}
% {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "8", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "4144.968000", "searching_seconds": "3664.106000", "encoding_seconds": "24.362000", "total_seconds": "7833.436000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "0.000000"}
% {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3490.155000", "searching_seconds": "6116.855000", "encoding_seconds": "37.276000", "total_seconds": "9644.286000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "0.000000"}

% latest results with -t 8
% {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "8", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "717.989000", "searching_seconds": "447.829000", "encoding_seconds": "11.366000", "total_seconds": "1177.184000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "0.000000"}
% {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "8", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3670.649000", "searching_seconds": "1301.471000", "encoding_seconds": "24.460000", "total_seconds": "4996.580000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "0.000000"}
% {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "8", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "3846.790000", "searching_seconds": "2191.239000", "encoding_seconds": "37.632000", "total_seconds": "6075.661000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "0.000000"}

&& 2389 (2124) & 3.07 & 83
&& 9754 (8876) & 2.96 & 119
&& 11298 (10107) & 2.91 & 91 \\

{\pth} (PC, $\alpha=0.94$, $c=7.0$)

&& 2389 (2117) & 2.61 & 101
&& 9754 (8857) & 2.58 & 172
&& 11298 (10077) & 2.56 & 142 \\

{\pth} (EF, $\alpha=0.94$, $c=7.0$)

&& 2389 (2118) & 2.36 & 187
&& 9754 (8860) & 2.32 & 215
&& 11298 (10082) & 2.31 & 207 \\

% =======
% && 2100 & 3.07 & 83
% % {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "557.798000", "searching_seconds": "1498.549000", "encoding_seconds": "11.023000", "total_seconds": "2067.370000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "85.628975"}
% % {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "551.323000", "searching_seconds": "1563.625000", "encoding_seconds": "9.205000", "total_seconds": "2124.153000", "pt_bits_per_key": "2.651774", "mapper_bits_per_key": "0.416224", "bits_per_key": "3.067997", "nanosec_per_key": "82.971686"}

% && 8880 & 2.96 & 120
% % {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "4441.349000", "searching_seconds": "4411.728000", "encoding_seconds": "23.258000", "total_seconds": "8876.335000", "pt_bits_per_key": "2.547078", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.963301", "nanosec_per_key": "119.173975"}


% && 10000 & 2.91 & 91 \\
% % {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "2100.912000", "searching_seconds": "6986.289000", "encoding_seconds": "35.983000", "total_seconds": "9123.184000", "pt_bits_per_key": "2.498342", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "110.384842"}
% % {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "2809.005000", "searching_seconds": "7262.232000", "encoding_seconds": "36.167000", "total_seconds": "10107.404000", "pt_bits_per_key": "2.498343", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.914566", "nanosec_per_key": "90.658567"}

% {\pth} (PC, $\alpha=0.94$, $c=7.0$)

% && 2100 & 2.61 & 101
% % {"n": "1983291944", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "551.323000", "searching_seconds": "1563.625000", "encoding_seconds": "1.605000", "total_seconds": "2116.553000", "pt_bits_per_key": "2.198462", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.614686", "nanosec_per_key": "100.842904"}

% && 8880 & 2.58 & 172
% % {"n": "4780950911", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "4441.349000", "searching_seconds": "4411.728000", "encoding_seconds": "3.856000", "total_seconds": "8856.933000", "pt_bits_per_key": "2.163938", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.580161", "nanosec_per_key": "171.829356"}

% && 10000 & 2.56 & 142 \\
% % {"n": "7384478110", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "1234567890", "num_threads": "1", "external_memory": "true", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "2809.005000", "searching_seconds": "7262.232000", "encoding_seconds": "5.775000", "total_seconds": "10077.012000", "pt_bits_per_key": "2.148619", "mapper_bits_per_key": "0.416224", "bits_per_key": "2.564842", "nanosec_per_key": "142.213669"}
% >>>>>>> f345813e4a58e00e4b7caa5e436648246c268972

\midrule

EMPHF
&& 4021 & 2.61 & 207
%after: && 4625 & 2.61 & 207
%before: && 2940 & {2.61} & {208}
&& 24862 & 2.61 & 231
%after: && 28008 & 2.61 & 232
%before: && 21716 & {2.61} & {229}
&& 37731 & 2.61 & 220 \\
%before: && \rob{37255} & {2.61} & {220}

\midrule

GOV
&& 2678 & 2.23 & 192
&& 8228 & 2.23 & 232
&& 10782 & 2.23 & 242 \\

\midrule

BBHash ($\gamma=1.0$)
&& 4750 & 3.07 & 294
&& 19360 & 3.07 & 320
&& 20178 & 3.07 & 305 \\

BBHash ($\gamma=2.0$)
&& 2365 & 3.71 & 217
&& 11074 & 3.71 & 236
&& 10254 & 3.71 & 235 \\

\bottomrule
\end{tabular}

==> tables/ext_mem_original.tex <==
% !TEX root = ../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c rlcc c rlcc c rlcc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{4}{c}{TweetsKB IDs}
&& \multicolumn{4}{c}{ClueWeb09-Full URLs}
&& \multicolumn{4}{c}{GoogleBooks 3-gr} \\

\cmidrule(lr){3-6}
\cmidrule(lr){7-12}
\cmidrule(lr){13-16}

&& \multicolumn{2}{c}{construction} & space & lookup
&& \multicolumn{2}{c}{construction} & space & lookup
&& \multicolumn{2}{c}{construction} & space & lookup \\

&& \multicolumn{2}{c}{(\secs)} & ({\bpk}) & ({\nspk})
&& \multicolumn{2}{c}{(\secs)} & ({\bpk}) & ({\nspk})
&& \multicolumn{2}{c}{(\secs)} & ({\bpk}) & ({\nspk}) \\

\midrule

{\pth} (D-D)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 2105 & (1058) & 3.07 & 80
&& 7234 & (4869) & 2.96 & 120
&& 9770 & (5865) & 2.91 & 91 \\
% && 2155 & (1022) & 3.07 & 82
% && 7333 & (4600) & 2.96 & 120
% && 9930 & (5406) & 2.91 & 91 \\

{\pth} (PC)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 2098 & (1051) & 2.61 & 101
&& 7161 & (4859) & 2.58 & 175
&& 9756 & (5736) & 2.56 & 143 \\
% && 2147 & (1015) & 2.61 & 102
% && 7314 & (4581) & 2.58 & 172
% && 9899 & (5375) & 2.56 & 142 \\

{\pth} (EF)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 2098 & (1052) & 2.36 & 188
&& 7225 & (4788) & 2.32 & 214
&& 9649 & (5849) & 2.31 & 208 \\
% && 2148 & (1016) & 2.36 & 188
% && 7318 & (4585) & 2.32 & 214
% && 9906 & (5381) & 2.31 & 207 \\

\midrule

{\pth-HEM} (D-D)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 989 & (581) & 2.85 & 116
&& 4651 & (3632) & 2.75 & 152
&& 5215 & (3510) & 2.71 & 135 \\

{\pth-HEM} (PC)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 982 & (580) & 2.61 & 128
&& 4522 & (3541) & 2.58 & 192
&& 5015 & (3366) & 2.57 & 190 \\

{\pth-HEM} (EF)%, $\alpha\text{=}0.94$, $c\text{=}7.0$)
&& 983 & (580) & 2.36 & 201
&& 4627 & (3631) & 2.32 & 235
&& 5179 & (3512) & 2.31 & 230 \\

\midrule

EMPHF
&& 4021 & & 2.61 & 207
%after: && 4625 & 2.61 & 207
%before: && 2940 & 2.61 & 208
&& 24862 & & 2.61 & 231
%after: && 28008 & 2.61 & 232
%before: && 21716 & 2.61 & 229
&& 37731 & & 2.61 & 220 \\
%before: && \rob{37255} & 2.61 & 220

%\midrule

EMPHF-HEM
&& 909 & & 3.03 & 279
%before: & 1204 & 3.03 & 279 \\
&& 3980 & & 3.31 & 304
%before: & 6853 & 3.31 & 304 \\
&& 5606 & & 3.06 & 304 \\
%before: & 6971 & 3.06 & 311 \\

\midrule

GOV
&& 2678 & (1463) & 2.23 & 192
&& 8228 & (5400) & 2.23 & 232
&& 10782 & (6461) & 2.23 & 242 \\

\midrule

BBHash ($\gamma=1.0$)
&& 4750 & (931) & 3.07 & 294
&& 19360 & (18391) & 3.07 & 320
&& 20178 & (9554) & 3.07 & 305 \\

BBHash ($\gamma=2.0$)
&& 2365 & (590) & 3.71 & 217
&& 11074 & (10348) & 3.71 & 236
&& 10254 & (5404) & 3.71 & 235 \\

\bottomrule
\end{tabular}

==> tables/int_mem/PTHash_partitioned_smaller_c.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{3pt}
\begin{tabular}{
c c ccc c ccc c ccc}

\toprule

\multirow{4}{*}{Compressor}

&& \multicolumn{3}{c}{UK2005 URLs, $c=3.1$}
&& \multicolumn{3}{c}{ClueWeb09-B URLs, $c=3.1$}
&& \multicolumn{3}{c}{GoogleBooks 2-gr, $c=3.6$} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

% /home/tranir/pt_hash/build/build 39459925 3.1 0.98 all -s 1234567890 -i /data2/urls/uk-2005.urls -p 8 -t 8 --check --lookup
% /home/tranir/pt_hash/build/build 49937704 3.1 0.98 all -s 1234567890 -i /data2/urls/cw09b.urls -p 16 -t 8 --check --lookup
% /home/tranir/pt_hash/build/build 665752080 3.6 0.98 all -s 1234567890 -i /data2/textual_collections/google_books/GoogleBooks.2-grams -p 128 -t 8 --check --lookup

D-D
&& 41  & 2.20 & 46
&& 54  & 2.24 & 49
&& 704 & 2.28 & 78 \\

PC
&& 41  & 2.11 & 45
&& 54  & 2.12 & 47
&& 704 & 2.11 & 73 \\

EF
&& 41  & 1.97 & 59
&& 54  & 1.97 & 61
&& 704 & 1.97 & 133 \\

\bottomrule
\end{tabular}


==> tables/int_mem/PTHash_partitioned_smaller_cv2.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{3pt}
\begin{tabular}{
c c ccc c ccc c ccc}

\toprule

\multirow{4}{*}{Compressor}

&& \multicolumn{3}{c}{UK2005 URLs, $c=3.8$}
&& \multicolumn{3}{c}{ClueWeb09-B URLs, $c=3.8$}
&& \multicolumn{3}{c}{GoogleBooks 2-gr, $c=3.9$} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

% /home/tranir/pt_hash/build/build 39459925 3.8 0.98 all -s 1234567890 -i /data2/urls/cw09 -p 8 -t 8 --check --lookup
% /home/tranir/pt_hash/build/build 49937704 3.8 0.98 all -s 1234567890 -i /data2/urls/cw09b.urls -p 16 -t 8 --check --lookup
% /home/tranir/pt_hash/build/build 665752080 3.9 0.98 all -s 1234567890 -i /data2/textual_collections/google_books/GoogleBooks.2-grams -p 128 -t 8 --check --lookup

D-D
&&  10 & 2.29 & 43
&&  13 & 2.29 & 48
&& 397 & 2.23 & 74 \\

PC
&&  10 & 2.20 & 44
&&  13 & 2.19 & 48
&& 397 & 2.14 & 73 \\

EF
&&  10 & 2.04 &  56
&&  13 & 2.04 &  59
&& 397 & 1.99 & 134 \\

\bottomrule
\end{tabular}



==> tables/int_mem/PTHash_single.tex <==
%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & construction & space & lookup \\

& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

UK2005 URLs
& 9 & 3.19 & 48 \\

\textcolor{blue}{(PC)}
& \textcolor{blue}{9} & \textcolor{blue}{2.81} & \textcolor{blue}{49} \\
% {"n": "39459925", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "false", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "4.219000", "searching_seconds": "4.915000", "encoding_seconds": "0.034000", "total_seconds": "9.168000", "pt_bits_per_key": "2.398674", "mapper_bits_per_key": "0.416243", "bits_per_key": "2.814917", "nanosec_per_key": "48.881761"}

ClueWeb09-B URLs
& 12 & 3.15 & 49 \\

\textcolor{blue}{(PC)}
& \textcolor{blue}{12} & \textcolor{blue}{2.80} & \textcolor{blue}{52} \\
% {"n": "49937704", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "false", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "5.388000", "searching_seconds": "6.581000", "encoding_seconds": "0.043000", "total_seconds": "12.012000", "pt_bits_per_key": "2.383756", "mapper_bits_per_key": "0.416239", "bits_per_key": "2.799995", "nanosec_per_key": "52.212200"}

GoogleBooks 2-gr
& 430 & 3.04 & 63 \\

\textcolor{blue}{(PC)}
& \textcolor{blue}{430} & \textcolor{blue}{2.66} & \textcolor{blue}{69} \\
% {"n": "665752080", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "1", "seed": "825878", "num_threads": "1", "external_memory": "false", "partitioning_seconds": "0.000000", "mapping_ordering_seconds": "73.898000", "searching_seconds": "347.494000", "encoding_seconds": "0.550000", "total_seconds": "421.942000", "pt_bits_per_key": "2.248655", "mapper_bits_per_key": "0.416225", "bits_per_key": "2.664880", "nanosec_per_key": "69.272823"}

\bottomrule
\end{tabular}


==> tables/int_mem/overall.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c ccc c ccc c ccc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{3}{c}{UK2005 URLs}
&& \multicolumn{3}{c}{ClueWeb09-B URLs}
&& \multicolumn{3}{c}{GoogleBooks 2-gr} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

{\pth} (D-D, $\alpha=0.94$, $c=7.0$)
&& 9 (5) & 3.11 & 47
&& 12 (6) & 3.07 & 49
&& 403 (154) & 2.97 & 63 \\

{\pth} (PC, $\alpha=0.94$, $c=7.0$)
&& 9 (4) & 2.82 & 49
&& 11 (6) & 2.80 & 52
&& 400 (151) & 2.67 & 69 \\

{\pth} (EF, $\alpha=0.94$, $c=7.0$)
&& 9 (4) & 2.50 & 59
&& 12 (6) & 2.49 & 63
&& 401 (152) & 2.38 & 121 \\

\midrule


{\pth-HEM} (D-D, $\alpha=0.94$, $c=7.0$)
&& {\e} (2) & 3.11 & 53
&& {\e} (3) & 3.08 & 57
&& {\e} (35) & 2.96 & 73 \\

{\pth-HEM} (PC, $\alpha=0.94$, $c=7.0$)
&& {\e} (2) & 2.82 & 55
&& {\e} (3) & 2.80 & 59
&& {\e} (35) & 2.67 & 83 \\

{\pth-HEM} (PC, $\alpha=0.94$, $c=7.0$)
&& {\e} ({\e}) & {\e} & {\e}
&& {\e} ({\e}) & {\e} & {\e}
&& {\e} ({\e}) & {\e} & {\e} \\

\midrule

FCH ($c=3.0$)
&& {1138} & {3.00} & {52}
&& {1438} & {3.00} & {55}
&& {--} & {--} & {--} \\

FCH ($c=4.0$)
&& 266 & 4.00 & 60
&& 267 & 4.00 & 64
&& 9110 & 4.00 & 54 \\

FCH ($c=5.0$)
&& {119} & {5.00} & {68}
&& {107} & {5.00} & {71}
&& {3225} & {5.00} & {55} \\

\midrule

CHD ($\lambda=4$)
&& 32 & 2.17 & 170
&& 43 & 2.17 & 185
&& 1251 & 2.17 & 410 \\

CHD ($\lambda=5$)
&& {84} & {2.07} & {173}
&& {115} & {2.07} & {182}
&& {3923} & {2.07} & {410} \\

CHD ($\lambda=6$)
&& {306} & {2.01} & {173}
&& {429} & {2.01} & {178}
&& {15583} & {2.01} & {406} \\

\midrule

EMPHF
&& 10 & 2.61 & 111
&& 13 & 2.61 & 138
&& 276 & 2.61 & 211 \\

\midrule

GOV
&& 39 (14) & 2.23 & 87
&& 47 (15) & 2.23 & 94
&& 613 (170) & 2.23 & 170 \\

\midrule

BBHash ($\gamma=1.0$)
&& 50 (12) & 3.10 & 154
% /home/tranir/BBHash/BootestFile /data2/urls/uk-2005.urls 1 1
%prima era  33, 3.09, 101
&& 66 (14) & 3.06 & 174
% /home/tranir/BBHash/BootestFile /data2/urls/cw09B_unique_url_shuffled.txt 1 1
%prima era  43, 3.06, 118
&& 1248 (189) & 3.08 & 273 \\
% /home/tranir/BBHash/BootestFile /data2/textual_collections/google_books/GoogleBooks.2-grams 1 1
%prima era  2037, 3.06, 203

BBHash ($\gamma=2.0$)
&& 31 (7) & 3.71 & 133
% /home/tranir/BBHash/BootestFile /data2/urls/uk-2005.urls 2 1
%prima era  26, 4.32, 101
&& 40 (9) & 3.71 & 150
% /home/tranir/BBHash/BootestFile /data2/urls/cw09B_unique_url_shuffled.txt 2 1
%prima era  35, 3.81, 114
&& 666 (102) & 3.71 & 204 \\
% /home/tranir/BBHash/BootestFile /data2/textual_collections/google_books/GoogleBooks.2-grams 2 1
%prima era  1395, 3.71, 159

\midrule

RecSplit ($\ell=5$, $b=5$)
&& {6} & {2.95} & {153}
&& {8} & {2.95} & {148}
&& {132} & {2.95} & {244} \\

RecSplit ($\ell=8$, $b=100$)
&& 37 & 1.79 & 113
&& 47 & 1.79 & 118
&& 724 & 1.80 & 202 \\

RecSplit ($\ell=12$, $b=9$)
&& {225} & {2.23} & {93}
&& {284} & {2.23} & {107}
&& {3789} & {2.23} & {225} \\


\bottomrule
\end{tabular}

==> tables/int_mem/partitioned.tex <==
% !TEX root = ../../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
l c ccc c ccc c ccc}

\toprule

\multirow{3}{*}{Method}

&& \multicolumn{3}{c}{UK2005 URLs}
&& \multicolumn{3}{c}{ClueWeb09-B URLs}
&& \multicolumn{3}{c}{GoogleBooks 2-gr} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}

&& construction & space & lookup
&& construction & space & lookup
&& construction & space & lookup \\

&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})}
&& {(\secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

{\pth} (D-D, $\alpha=0.94$, $c=7.0$)

&& 2 & 3.11 & 53
% ./build 39459925 7.0 0.94 dictionary_dictionary -s 825878 --verbose -i /data2/urls/uk-2005.urls -p 8 -t 8
% {"n": "39459925", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "8", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "0.782000", "mapping_ordering_seconds": "0.608000", "searching_seconds": "0.617000", "encoding_seconds": "0.039000", "total_seconds": "2.046000", "pt_bits_per_key": "2.693400", "mapper_bits_per_key": "0.416382", "bits_per_key": "3.109782", "nanosec_per_key": "53.062726"}

&& 3 & 3.08 & 57
% ./build 49937704 7.0 0.94 dictionary_dictionary -s 825878 --verbose -i /data2/urls/cw09B_unique_url_shuffled.txt -p 16 -t 8
% {"n": "49937704", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "16", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "0.990000", "mapping_ordering_seconds": "0.730000", "searching_seconds": "0.742000", "encoding_seconds": "0.055000", "total_seconds": "2.517000", "pt_bits_per_key": "2.659145", "mapper_bits_per_key": "0.416479", "bits_per_key": "3.075624", "nanosec_per_key": "57.377529"}

&& 35 & 2.96 & 73 \\
% ./build 665752080 7.0 0.94 dictionary_dictionary -s 825878 --verbose -i /data2/textual_collections/google_books/GoogleBooks.2-grams -p 128 -t 8
% {"n": "665752080", "c": "7.000000", "alpha": "0.940000", "encoder_type": "dictionary-dictionary", "num_partitions": "128", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "8.116000", "mapping_ordering_seconds": "9.503000", "searching_seconds": "16.148000", "encoding_seconds": "0.569000", "total_seconds": "34.336000", "pt_bits_per_key": "2.539585", "mapper_bits_per_key": "0.416380", "bits_per_key": "2.955965", "nanosec_per_key": "73.159272"}


{\pth} (PC, $\alpha=0.94$, $c=7.0$)

&& 2 & 2.82 & 55
% ./build 39459925 7.0 0.94 partitioned_compact -s 825878 --verbose -i /data2/urls/uk-2005.urls -p 8 -t 8
% {"n": "39459925", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "8", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "0.831000", "mapping_ordering_seconds": "0.605000", "searching_seconds": "0.624000", "encoding_seconds": "0.007000", "total_seconds": "2.067000", "pt_bits_per_key": "2.399062", "mapper_bits_per_key": "0.416382", "bits_per_key": "2.815445", "nanosec_per_key": "54.799811"}

&& 3 & 2.80 & 59
% ./build 49937704 7.0 0.94 partitioned_compact -s 825878 --verbose -i /data2/urls/cw09B_unique_url_shuffled.txt -p 16 -t 8
% {"n": "49937704", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "16", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "1.086000", "mapping_ordering_seconds": "0.722000", "searching_seconds": "0.737000", "encoding_seconds": "0.009000", "total_seconds": "2.554000", "pt_bits_per_key": "2.384804", "mapper_bits_per_key": "0.416479", "bits_per_key": "2.801283", "nanosec_per_key": "59.163538"}

&& 35 & 2.67 & 83 \\
% ./build 665752080 7.0 0.94 partitioned_compact -s 825878 --verbose -i /data2/textual_collections/google_books/GoogleBooks.2-grams -p 128 -t 8
% {"n": "665752080", "c": "7.000000", "alpha": "0.940000", "encoder_type": "partitioned_compact", "num_partitions": "128", "seed": "825878", "num_threads": "8", "external_memory": "false", "partitioning_seconds": "9.493000", "mapping_ordering_seconds": "9.085000", "searching_seconds": "16.769000", "encoding_seconds": "0.095000", "total_seconds": "35.442000", "pt_bits_per_key": "2.248940", "mapper_bits_per_key": "0.416380", "bits_per_key": "2.665320", "nanosec_per_key": "83.199660"}


\midrule

GOV
&& {14} & {2.23} & {87}
&& {15} & {2.23} & {94}
&& {170} & {2.23} & {170} \\

\midrule

BBHash ($\gamma=1.0$)
&& 12 & 3.06 & 155
% /home/tranir/BBHash/BootestFile /data2/urls/uk-2005.urls 1 8
&& 14 & 3.06 & 173
% /home/tranir/BBHash/BootestFile /data2/urls/cw09B_unique_url_shuffled.txt 1 8
&& 189 & 3.08 & 276 \\
% /home/tranir/BBHash/BootestFile /data2/textual_collections/google_books/GoogleBooks.2-grams 1 8

BBHash ($\gamma=2.0$)
&& 7 & 3.71 & 135
% /home/tranir/BBHash/BootestFile /data2/urls/uk-2005.urls 2 8
&& 9 & 3.71 & 152
% /home/tranir/BBHash/BootestFile /data2/urls/cw09B_unique_url_shuffled.txt 2 8
&& 102 & 3.71 & 204 \\
% /home/tranir/BBHash/BootestFile /data2/textual_collections/google_books/GoogleBooks.2-grams 2 8


\bottomrule
\end{tabular}

==> tables/methods.tex <==
% !TEX root = ../paper.tex
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l c cc}

\toprule

\multirow{2}{*}{Method}
&&
\multicolumn{2}{c}{Implementation} \\

\cmidrule(lr){3-4}

&& multi-threading & external memory \\

\midrule

{\pth}      && $\checkmark$ & $\checkmark$ \\
{\pth-HEM}  && $\checkmark$ & $\checkmark$ \\

% \cmidrule(lr){1-4}

FCH~\cite{fox1992faster}                   &&              &              \\
CHD~\cite{belazzougui2009hash}             &&              &              \\
EMPHF~\cite{belazzougui2014cache}          &&              & $\checkmark$ \\
EMPHF-HEM~\cite{belazzougui2014cache}      &&              & $\checkmark$ \\
GOV~\cite{genuzio2016fast,genuzio2020fast} && $\checkmark$ & $\checkmark$ \\
BBHash~\cite{limasset2017fast}             && $\checkmark$ & $\checkmark$ \\
RecSplit~\cite{esposito2020recsplit}       &&              &              \\

\bottomrule
\end{tabular}

==> tables/overall.tex <==
% !TEX root = ../paper.tex
\setlength{\tabcolsep}{1pt}
\begin{tabular}{
l c
%ccc c ccc c
ccc c ccc}

\toprule

\multirow{3}{*}{Method}
%&& \multicolumn{3}{c}{{$n=10^6$}}
%&& \multicolumn{3}{c}{{$n=10^7$}}
&& \multicolumn{3}{c}{{$n=10^8$}}
&& \multicolumn{3}{c}{{$n=10^9$}} \\

%\cmidrule(lr){3-17}
\cmidrule(lr){3-5}
\cmidrule(lr){7-9}

%&& constr. & space & lookup
%&& constr. & space & lookup
&& constr. & space & lookup
&& constr. & space & lookup \\

%&& [secs] & [{\bpk}] & [{\nspk}]
%&& [secs] & [{\bpk}] & [{\nspk}]
&& ({\secs}) & ({\bpk}) & ({\nspk})
&& ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

%\cmidrule(lr){1-1}
%\cmidrule(lr){3-5}
%\cmidrule(lr){7-9}
%\cmidrule(lr){11-13}
%\cmidrule(lr){15-17}

FCH, $c=3$
%    && {1.445} & {3.00} & {10}
%    && {121} & {3.00} & {11}
    && {4286} & {3.00} & {30}
    && {---} & {---} & {---} \\
FCH, $c=4$
%    && {0.513} & {4.00} & {10}
%    && {20} & {4.00} & {11}
    && {463} & {4.00} & {30}
    && {15904} & {4.00} & {35} \\
FCH, $c=5$
%    && {0.286} & {5.00} & {10}
%    && {12} & {5.00} & {11}
    && {145} & {5.00} & {30}
    && {2937} & {5.00} & {35} \\
FCH, $c=6$
%    && {0.258} & {6.00} & {10}
%    && {7} & {6.00} & {11}
    && {81} & {6.00} & {30}
    && {2133} & {6.00} & {35} \\
FCH, $c=7$
%	&& {0.173} & {7.00} & {10}
%    && {6} & {7.00} & {11}
    && {68} & {7.00} & {30}
    && {1221} & {7.00} & {35} \\

\midrule
%\cmidrule(lr){1-1}
%\cmidrule(lr){3-5}
%\cmidrule(lr){7-9}
%\cmidrule(lr){11-13}
%\cmidrule(lr){15-17}

CHD, $\lambda=4$
%    && {0.441} & {2.17} & {88}
%    && {5.933} & {2.17} & {115}
    && {121} & {2.17} & {204}
    && {1972} & {2.17} & {419} \\
CHD, $\lambda=5$
%    && {1.338} & {2.07} & {88}
%    && {16.48} & {2.07} & {116}
    && {358} & {2.07} & {204}
    && {5964} & {2.07} & {417} \\
CHD, $\lambda=6$
%    && {5.282} & {2.01} & {90}
%    && {63.21} & {2.01} & {116}
    && {1418} & {2.01} & {197}
    && {23746} & {2.01} & {416} \\

\midrule


EMPHF
%    && {0.149} & {2.61} & {51}
%    && {2.272} & {2.61} & {58}
    && {24} & {2.61} & {147}
    && {374} & {2.61} & {199} \\

%EMPHF HEM
%    && {0.161} & {3.15} & {57}
%    && {1.789} & {3.47} & {69}
%    && {20} & {3.30} & {163}
%    && {210} & {3.16} & {271} \\

\midrule

GOV
    && 85 & 2.23 & 110
    && 875 & 2.23 & 175 \\

\midrule

BBHash, $\gamma=1$
%    && {-} & {3.06} & {36}
%    && {-} & {3.06} & {42}
    && {14} & {3.06} & {119}
    && {253} & {3.06} & {170} \\
BBHash, $\gamma=2$
%    && {-} & {3.71} & {32}
%    && {-} & {3.71} & {36}
    && {10} & {3.71} & {108}
    && {152} & {3.71} & {143} \\
BBHash, $\gamma=5$
%    && {-} & {6.87} & {27}
%    && {-} & {6.87} & {32}
    && {8} & {6.87} & {98}
    && {100} & {6.87} & {113} \\

\midrule


RecSplit, $\ell$=5, $b$=5
%    && {0.132} & {2.95} & {57}
%    && {1.466} & {2.95} & {68}
    && {20} & {2.95} & {157}
    && {233} & {2.95} & {220} \\
RecSplit, $\ell$=8, $b$=100
%    && {0.908} & {1.79} & {72}
%    && {9.148} & {1.79} & {81}
    && {92} & {1.80} & {124}
    && {936} & {1.80} & {204} \\
RecSplit, $\ell$=12, $b$=9
%    && {5.634} & {2.24} & {46}
%    && {56.839} & {2.23} & {56}
    && {569} & {2.23} & {110}
    && {5700} & {2.23} & {197} \\

\midrule

{\pth} && & & && & & \\

(i) C-C, $\alpha$=0.99, $c$=7
    && 42 & 3.25 & 28
    && 1042 & 3.14 & 37 \\
(ii) D-D, $\alpha$=0.88, $c$=11
    && 19 & 4.05 & 46
    && 308 & 4.05 & 64 \\
(iii) EF, $\alpha$=0.99, $c$=6
    && 45 & 2.26 & 49
    && 1799 & 2.17 & 101 \\

%\cmidrule(lr){2-9}

(iv) D-D, $\alpha$=0.94, $c$=7
    && 26 & 3.23 & 37
    && 689 & 2.99 & 55 \\




\bottomrule
\end{tabular}


==> tables/perf_competitors_variable_length_keys.tex <==

\setlength{\tabcolsep}{2pt}

\begin{tabular}{
l
c ccc c ccc
c ccc c ccc}

\toprule

\multirow{5}{*}{Method}
&& \multicolumn{3}{c}{GoogleBooks 1-gr}
&& \multicolumn{3}{c}{GoogleBooks 2-gr}
&& \multicolumn{3}{c}{ClueWeb09 URLs}
&& \multicolumn{3}{c}{UK2005 URLs} \\

&& \multicolumn{3}{c}{$n=\num{24357349}$}
&& \multicolumn{3}{c}{$n=\num{665752080}$}
&& \multicolumn{3}{c}{$n=\num{49937704}$}
&& \multicolumn{3}{c}{$n=\num{39459925}$} \\

&& \multicolumn{3}{c}{avg. key length $10.29$}
&& \multicolumn{3}{c}{avg. key length $17.21$}
&& \multicolumn{3}{c}{avg. key length $54.72$}
&& \multicolumn{3}{c}{avg. key length $71.37$} \\

\cmidrule(lr){3-5}
\cmidrule(lr){7-9}
\cmidrule(lr){11-13}
\cmidrule(lr){15-17}

&& constr. & space & lookup
&& constr. & space & lookup
&& constr. & space & lookup
&& constr. & space & lookup \\

&& {(secs)} & {({\bpk})} & {({\nspk})}
&& {(secs)} & {({\bpk})} & {({\nspk})}
&& {(secs)} & {({\bpk})} & {({\nspk})}
&& {(secs)} & {({\bpk})} & {({\nspk})} \\

\midrule

FCH, $c=3$
    && {417} & {3.00} & {20}
    && {-} & {3.00} & {-}
    && {1438} & {3.00} & {55}
    && {1138} & {3.00} & {52} \\
FCH, $c=4$
    && {81} & {4.00} & {21}
    && {9109} & {4.00} & {54}
    && {267} & {4.00} & {64}
    && {266} & {4.00} & {60} \\
FCH, $c=5$
    && {51} & {5.00} & {26}
    && {3225} & {5.00} & {55}
    && {107} & {5.00} & {71}
    && {119} & {5.00} & {68} \\
FCH, $c=6$
    && {32} & {6.00} & {29}
    && {1624} & {6.00} & {55}
    && {90} & {6.00} & {75}
    && {71} & {6.00} & {73} \\
FCH, $c=7$
	&& {20} & {7.00} & {32}
    && {1029} & {7.00} & {55}
    && {152} & {7.00} & {78}
    && {66} & {7.00} & {77} \\

\midrule

CHD, $\lambda=4$
    && {17} & {2.17} & {132}
    && {1251} & {2.17} & {407}
    && {43} & {2.17} & {185}
    && {32} & {2.17} & {170} \\
CHD, $\lambda=5$
    && {45} & {2.07} & {133}
    && {3923} & {2.07} & {410}
    && {115} & {2.07} & {182}
    && {84} & {2.07} & {173} \\
CHD, $\lambda=6$
    && {167} & {2.01} & {133}
    && {15583} & {2.01} & {406}
    && {429} & {2.01} & {178}
    && {306} & {2.01} & {173} \\

\midrule

BBHash, $\gamma=1$
    && {20} & {3.11} & {63}
    && {2037} & {3.06} & {203}
    && {43} & {3.06} & {118}
    && {33} & {3.09} & {101} \\
BBHash, $\gamma=2$
    && {15} & {3.88} & {55}
    && {1395} & {3.71} & {159}
    && {35} & {3.81} & {114}
    && {26} & {4.32} & {101} \\
BBHash, $\gamma=5$
    && {10} & {7.23} & {71}
    && {723} & {6.88} & {125}
    && {26} & {9.72} & {116}
    && {22} & {13.84} & {109} \\

\midrule

EMPHF
    && {5} & {2.61} & {70}
    && {276} & {2.61} & {211}
    && {13} & {2.61} & {138}
    && {10} & {2.61} & {111} \\
EMPHF HEM
   && {5} & {3.32} & {78}
   && {-} & {-} & {-}
   && {11} & {3.3} & {164}
   && {9} & {3.49} & {153} \\

\midrule


RecSplit, $\ell=5$, $b=5$
    && {4} & {3.32} & {85}
    && {132} & {2.95} & {244}
    && {8} & {2.95} & {148}
    && {6} & {2.95} & {153} \\
RecSplit, $\ell=8$, $b=100$
    && {23} & {1.80} & {96}
    && {724} & {1.80} & {202}
    && {47} & {1.79} & {118}
    && {37} & {1.79} & {113} \\
RecSplit, $\ell=12$, $b=9$
    && {138} & {2.23} & {70}
    && {3789} & {2.23} & {225}
    && {284} & {2.23} & {107}
    && {225} & {2.23} & {93} \\

\bottomrule
\end{tabular}


==> tables/perf_variable_length_keys.tex <==
% !TEX root = ../paper.tex


%GoogleBooks 1-grams   &  \,\,24,357,349 &  \,\,82.32 \\
%GoogleBooks 2-grams   &     665,752,080 &     137.68 \\
%ClueWeb09 URLs        &  \,\,49,937,704 &     437.76 \\
%UK2005 URLs           &  \,\,39,459,925 &     570.96 \\


%\setlength{\tabcolsep}{1pt}
\begin{tabular}{l cccc}

\toprule

\multirow{2}{*}{Collection} & avg. key size & constr. & space & lookup \\

& \small (bits) & ({\secs}) & ({\bpk}) & ({\nspk}) \\

\midrule

GoogleBooks 1-grams
& \,\,82.32 & 5 & 3.27 & 22 \\

64-bit keys
& \,\,64.00 & 5 & 3.27 & 16 \\

\midrule

GoogleBooks 2-grams
& 137.68 & 430 & 3.04 & 63 \\

64-bit keys
& \,\,64.00 & 428 & 3.04 & 54 \\

\midrule

ClueWeb09 URLs
& 437.76 & 12 & 3.15 & 49 \\

64-bit keys
& \,\,64.00 & 11 & 3.15 & 24 \\

\midrule

UK2005 URLs
& 570.96 & 9 & 3.19 & 48 \\

64-bit keys
& \,\,64.00 & 9 & 3.19 & 22 \\

\bottomrule
\end{tabular}

